Tandem Transformers for Inference Efficient LLMs

The autoregressive nature of conventional large language models (LLMs) inherently limits inference speed, as tokens are generated sequentially. While speculative and parallel decoding techniques attempt to mitigate this, they face limitations: either relying on less accurate smaller models for generation or failing to fully leverage the base LLM's representations. We introduce a novel architecture, Tandem transformers, to address these issues. This architecture uniquely combines (1) a small autoregressive model and (2) a large model operating in block mode (processing multiple tokens simultaneously). The small model's predictive accuracy is substantially enhanced by granting it attention to the large model's richer representations. On the PaLM2 pretraining dataset, a tandem of PaLM2-Bison and PaLM2-Gecko demonstrates a 3.3% improvement in next-token prediction accuracy over a standalone PaLM2-Gecko, offering a 1.16x speedup compared to a PaLM2-Otter model with comparable downstream performance. We further incorporate the tandem model within the speculative decoding (SPEED) framework where the large model validates tokens from the small model. This ensures that the Tandem of PaLM2-Bison and PaLM2-Gecko achieves substantial speedup (around 1.14x faster than using vanilla PaLM2-Gecko in SPEED) while maintaining identical downstream task accuracy.

==> disc-deeptandem.tex <==
\section{Conclusions and Discussion}\label{sec:conc}
In this work, we introduce a novel architecture, Tandem Transformers, which combines a small autoregressive model with a large model operating in block mode. Tandem Transformers substantially boost the small model's predictive accuracy by allowing it to attend to representations from the large model. In our experiments, a Tandem model comprising of \bison and \gecko substantially improves over a standalone \gecko, and gives comparable performance to the \otter model, while being $1.16 \times$ faster than the \otter model. When used within the SPEED setup as a secondary model, the distilled \emph{Tandem} \gecko model gives around $1.14 \times$ speedup over a distilled \gecko model. We further improve our Tandem model through an adaptive block length procedure in SPEED and obtain around $1.22 \times$ speedup over using \geckodistill as the secondary model.


\paragraph{Limitations and Future Directions}
\begin{itemize}
    \item \textbf{Other Variants of Tandem.} In our current approach, we use the large model only through its representations of the past tokens. Is it possible to use the large model to also generate a \emph{plan for the future $\gamma$ tokens} along the lines of deep Tandem Transformers?
    % Allow for non-auto-regressive generation through plan generation by the large model.
    \item \textbf{Alternative to LoRA for Finetuning.} The current approach for finetuning a base model for multiple downstream applications is through low rank adaptation (LoRA)~\cite{hu2021lora}. It will be interesting to explore whether Tandem with block length $0$ can be an effective alternative to LoRA, while reducing the training cost substantially since backpropagation needs to be done only for the small model.
    \item \textbf{Adaptive $\gamma$ for Larger \numsamples /batch-size.} While we see promising results with adaptive $\gamma$ in SPEED for num samples $1$, extending it to larger num samples seems challenging. Identifying an effective way of determining when to continue generating with small model vs verifying with large model, in the larger num samples setting, is also an interesting direction of future work.
    \item \textbf{Smaller Drafter Models in SPEED.} Finally, we hope that Tandem can enable using even smaller drafter models in SPEED, compared to the ones currently being pursued, leading to both memory as well as latency improvements.
    % Our current implementation of adaptive $\gamma$ for num-samples $>$ 1 involves continuing generation with the secondary model until and unless all the samples want to fall back to the primary model. However, by doing so, we are generating several unnecessary tokens for some sample that wants to exit early. This forces us to use a small $\gamma_{max}$, thus significantly reducing our gains. In future, we would like to refine our exit strategy to get latency gains for num-samples $>$ 1. 
\end{itemize}


==> experiments-deeptandem.tex <==
\subsection{Experimental Results for Deep Tandem Transformers}
In this section, we present preliminary experimental results on deep Tandem Transformers compared with the standard architecture. For this section, we consider the LaMDA models along with the training protocol as described in~\cite{thoppilan2022lamda}. In particular, we consider the 1B parameter model from the LaMDA family and construct a deep Tandem version of it by splitting the $16$ layers equally between $\Ml$ and $\Ms$ (so each of them has $8$ layers), and with block length $\gamma=2$. The results, presented in Table~\ref{tab:deep-Tandem} suggest that we suffer minimal loss by letting the autoregressive component be only a part of the entire model.
\input{tables/table6}
% \begin{table}[h]
% \begin{center}
% \begin{tabular}{| m{5em}  | m{5em} |}
%  \hline
%  LaMDA-1B & DeepTandem-LaMDA-1B \\ [1ex] 
%  \hline \hline
%  2.71 & 2.86 \\
%  \hline
% \end{tabular}
% \end{center}
% \caption{Pretraining log perplexity of a deep Tandem model compared with the original one with the same number of parameters.}
% \label{tab:deep-Tandem}
% \end{table}
\subsection{Importance of the Small Autoregressive Component}
In this section we present the log perplexity achieved by a block prediction model similar to~\cite{stern2018blockwise}, where we predict the next block of $\gamma =8$ tokens simultaneously. In other words, we directly train the output $\xss{i}{L_L}$ of the large model in Equation~\eqref{eqn:deep-Tandem-1} to predict the $i^\textrm{th}$ token $x\left[i\right]$. The CE loss of the resulting model, and its comparison with a fully autoregressive model is presented in Table~\ref{tab:block-ahead}. As we can see, the cross entropy loss of such a model is much higher compared to that of the original model, which is fully autoregressive.
\input{tables/table7}


==> intro-deeptandem.tex <==
\paragraph{}
Finally, we also present a variant of the Tandem architecture, where the large model produces a sketch of the next block of tokens, which is then passed on to the small model, along with the previous tokens in the current block, and the small model then predicts next token autoregressively. We refer to this architecture as \emph{deep Tandem} Transformers. Preliminary results suggest that even a small model can accurately capture the effect of the most recent tokens while a large model is able to produce an effective sketch of the next block of tokens.


==> related_deeptandem.tex <==
\paragraph{Block parallel decoding}: Another very related line of work to deep Tandem Transformers is the idea of block parallel decoding~\cite{stern2018blockwise}, where instead of using the final layer representation to predict only the next token, the model uses multiple heads to predict the next block of say $\gamma$ tokens. However, these models lose quite a bit of accuracy since we are trying to predict multiple tokens ahead without seeing all the tokens thus far. Deep Tandem Transformers addresses this issue by retaining a small model to do fully autoregressive prediction where we condition on all the tokens seen so far.

==> tables/table6.tex <==
\begin{table}[h]
% \begin{center}
\caption{Accuracy and CE loss of Tandem model with respect to ground truth labels on the pretraining data.}
\centering
\vspace{2mm}
\begin{tabular}{lcc}
 \toprule
 & Topline & Tandem \\
 \midrule
 Accuracy & 45.1 & 43.3 \\ 
 % \midrule
 CE loss & 2.71 & 2.85 \\
 % \midrule
 Speedup estimate & $1 \times$ & $1.25 \times$ \\ 
 \bottomrule
\end{tabular}
% \end{center}
\label{tab:deep-Tandem}
\end{table}

==> tables/table7.tex <==
\begin{table}[h]
% \begin{center}
\caption{Pretraining log perplexity of an autoregressive 
 model compared to a block prediction model with block length $\gamma=8$. Both models are taken to have the same architecture as LaMDA-1B, except for the difference between block prediction and autoregressive prediction.}
 \vspace{2mm}
\centering
\begin{tabular}{cc}
 \toprule
 Autoregressive & $8$-Block prediction \\ [1ex] 
 \midrule
 2.71 & 5.55 \\
 \bottomrule
\end{tabular}
% \end{center}
\label{tab:block-ahead}
\end{table}

